Boosting Masked ECG-Text Auto-Encoders as Discriminative Learners

The accurate interpretation of Electrocardiogram (ECG) signals is pivotal for diagnosing cardiovascular diseases. Integrating ECG signals with accompanying textual reports further holds immense potential to enhance clinical diagnostics by combining physiological data and qualitative insights. However, this integration faces significant challenges due to inherent modality disparities and the scarcity of labeled data for robust cross-modal learning. To address these obstacles, we propose D-BETA, a novel framework that pre-trains ECG and text data using a contrastive masked auto-encoder architecture. D-BETA uniquely combines the strengths of generative with boosted discriminative capabilities to achieve robust cross-modal representations. This is accomplished through masked modality modeling, specialized loss functions, and an improved negative sampling strategy tailored for cross-modal alignment. Extensive experiments on five public datasets across diverse downstream tasks demonstrate that D-BETA significantly outperforms existing methods, achieving an average AUC improvement of 15% in linear probing with only one percent of training data and 2% in zero-shot performance without requiring training data over state-of-the-art models. These results highlight the effectiveness of D-BETA, underscoring its potential to advance automated clinical diagnostics through multi-modal representations. Our sample code and checkpoint are made available at https://github.com/manhph2211/D-BETA.

==> tables/hidden_dim.tex <==
\setlength{\tabcolsep}{1.5pt}
\centering
\scriptsize
\caption{Effects of hidden dimension from encoder's embedding.} 
\label{tab:system_performance}
\vspace{-0.5em}
\begin{tabular}{lccc}
\toprule
\textbf{Embedding dim} & \textbf{Full fine-tune} & \textbf{Linear probing} & \textbf{Zero-shot} \\
\midrule
768 & \textbf{81.88 $\pm$ 3.52}  & \textbf{80.52 $\pm$ 6.08} & \textbf{69.74$\pm$ 10.75} \\
\midrule
256 & -- & -- & -- \\
64& -- & -- & -- \\
\bottomrule
\end{tabular}
